CLUTRR: A Diagnostic Benchmark for Inductive Reasoning from Text

The recent success of natural language understanding (NLU) systems has been troubled by results highlighting the failure of these models to generalize in a systematic and robust way. In this work, we introduce a diagnostic benchmark suite, named CLUTRR, to clarify some key issues related to the robustness and systematicity of NLU systems. Motivated by classic work on inductive logic programming, CLUTRR requires that an NLU system infer kinship relations between characters in short stories. Successful performance on this task requires both extracting relationships between entities, as well as inferring the logical rules governing these relationships. CLUTRR allows us to precisely measure a model's ability for systematic generalization by evaluating on held-out combinations of logical rules, and it allows us to evaluate a model's robustness by adding curated noise facts. Our empirical results highlight a substantial performance gap between state-of-the-art NLU models (e.g., BERT and MAC) and a graph neural network model that works directly with symbolic inputs---with the graph-based model exhibiting both stronger generalization and greater robustness.

==> tables/table_data.tex <==
\begin{table*}[]
\caption{Various dataset variants of CLUTRR that are examined in this work.}
\label{tab:data_variants}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
Task & Variant name & Training Clause length $k$ & Testing Clause length $k$ \\ \midrule
Systematic Generalization & \texttt{CLUTRR-Gen} & $(2,3)$, $(2,3,4)$, & $(2,3, \ldots, 10)$ \\
Robust Reasoning - Training on clean data & \texttt{CLUTRR-AMT} & $(2,3)$ & $(2,3)$ \\
Robust Reasoning - Training on supporting facts & \texttt{CLUTRR-Supporting} & $(2,3)$ & $(2,3)$ \\
Robust Reasoning - Training on irrelevant facts & \texttt{CLUTRR-Irrelevant} & $(2,3)$ & $(2,3)$ \\
Robust Reasoning - Training on disconnected facts & \texttt{CLUTRR-Disconnected} & $(2,3)$ & $(2,3)$ \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> tables/table_data_example.tex <==
\begin{table*}[htb!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{2cm}|p{3cm}p{3cm}|p{1cm}p{1cm}|}
\hline
\multirow{2}{*}{Variant} & \multicolumn{2}{l}{Sample Story} & \multirow{2}{*}{Query} & \multirow{2}{*}{Target} \\ \cline{2-3}
 & \multicolumn{1}{l|}{CLUTRR-Toy} & CLUTRR &  &  \\ \hline
CLUTRR-Gen & 
[Stephanie] is a daughter of [Latoria]. [Carrie] is a sister of [Stephanie]. &
 [Latoria] wants to make a special meal for her daughter [Stephanie]'s birthday. [Carrie] needed to go to the store. [Carrie] asked her sister [Stephanie] for a ride.
\multicolumn{1}{l|}{}
  &
 ('Latoria', 'Carrie') &
 daughter \\
CLUTRR-Clean & \multicolumn{1}{l|}{}
  &
  &
  &
  \\
CLUTRR-Supporting & \multicolumn{1}{l|}{} 
  &
  &
  &
  \\
CLUTRR-Irrelevant & \multicolumn{1}{l|}{} 
  &
  &
  &
  \\
CLUTRR-Disconnected & \multicolumn{1}{l|}{} 
  &
  &
  &
  \\ \hline
\end{tabular}%
}
\caption{Examples of the CLUTRR Benchmark suite for various variants}
\label{tab:data_examples}
\end{table*}


==> tables/table_puzzles.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\tiny
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{4cm}|p{2.5cm}|p{2cm}|p{0.5cm}|p{1cm}|p{1cm}|p{1cm}@{}}
\toprule
\textbf{Puzzle} & \textbf{Question} & \textbf{Gender} & \textbf{Relation Length} & \textbf{Answer} & \textbf{Human Reported Difficulty} & \textbf{Mean Time taken} \\ \midrule
{[}Charles{]}'s son {[}Christopher{]} entered rehab for the ninth time at the age of thirty. {[}Randolph{]} had a nephew called {[}Christopher{]} who had n't seen for a number of years. & Randolph is the \_\_\_\_\_ of Charles & \begin{tabular}[c]{@{}l@{}}Charles:male,\\ Christopher:male,\\ Randolph:male\end{tabular} & 2 & brother & \multirow{3}{*}{1.488 +- 1.25} &  \\
{[}Randolph{]} and his sister {[}Sharon{]} went to the park. {[}Arthur{]} went to the baseball game with his son {[}Randolph{]} & Sharon is the \_\_\_\_\_ of Arthur & \begin{tabular}[c]{@{}l@{}}Arthur:male,\\ Randolph:male,\\ Sharon:female\end{tabular} & 2 & daughter &  &  \\
{[}Frank{]} went to the park with his father, {[}Brett{]}. {[}Frank{]} called his brother {[}Boyd{]} on the phone. He wanted to go out for some beers. & Brett is the \_\_\_\_\_ of Boyd & \begin{tabular}[c]{@{}l@{}}Boyd:male,\\ Frank:male,\\ Brett:male\end{tabular} & 2 & father &  &  \\ \midrule
{[}Roger{]} was playing baseball with his sons {[}Sam{]} and {[}Leon{]}. {[}Sam{]} had to take a break though because he needed to call his sister {[}Robin{]}. & Leon is the \_\_\_\_\_ of Robin & \begin{tabular}[c]{@{}l@{}}Robin:female,\\ Sam:male,\\ Roger:male,\\ Leon:male\end{tabular} & 3 & brother & \multirow{3}{*}{2.41 +- 1.33} &  \\
{[}Elvira{]} and her daughter {[}Nancy{]} went shopping together last Monday and they bought new shoes for {[}Elvira{]}'s kids. {[}Pedro{]} and his sister {[}Allison{]} went to the fair. {[}Pedro{]}'s mother, {[}Nancy{]}, was out with friends for the day. & Elvira is the \_\_\_\_\_ of Allison & \begin{tabular}[c]{@{}l@{}}Allison:female,\\ Pedro:male,\\ Nancy:female,\\ Elvira:female\end{tabular} & 3 & grandmother &  &  \\
{[}Roger{]} met up with his sister {[}Nancy{]} and her daughter {[}Cynthia{]} at the mall to go shopping together. {[}Cynthia{]}'s brother {[}Pedro{]} was going to be the star in the new show. & Pedro is the \_\_\_\_\_ of Roger & \begin{tabular}[c]{@{}l@{}}Roger:male,\\ Nancy:female,\\ Cynthia:female,\\ Pedro:male\end{tabular} & 3 & nephew &  &  \\ \midrule
{[}Celina{]} has been visiting her sister, {[}Fran{]} all week. {[}Fran{]} is also the daughter of {[}Bethany{]}. {[}Ronald{]} loves visiting his aunt {[}Bethany{]} over the weekends. {[}Samuel{]}'s son {[}Ronald{]} entered rehab for the ninth time at the age of thirty. & Celina is the \_\_\_\_\_ of Samuel & \begin{tabular}[c]{@{}l@{}}Samuel:male,\\ Ronald:male,\\ Bethany:female,\\ Fran:female,\\ Celina:female\end{tabular} & 4 & niece & \multirow{3}{*}{3.81 +- 1.46} &  \\
{[}Celina{]} adores her daughter {[}Bethany{]}. {[}Bethany{]} loves her very much, too. {[}Jackie{]} called her mother {[}Bethany{]} to let her know she will be back home soon. {[}Thomas{]} was helping his daughter {[}Fran{]} with her homework at home. Afterwards, {[}Fran{]} and her sister {[}Jackie{]} played Xbox together. & Celina is the \_\_\_\_\_ of Thomas & \begin{tabular}[c]{@{}l@{}}Thomas:male,\\ Fran:female,\\ Jackie:female,\\ Bethany:female,\\ Celina:female\end{tabular} & 4 & daughter &  &  \\
{[}Raquel{]} is {[}Samuel{]} 'daughter and they go shopping at least twice a week together. {[}Kenneth{]} and her mom, {[}Theresa{]}, had a big fight. {[}Theresa{]}'s son, {[}Ronald{]}, refused to get involved. {[}Ronald{]} was having an argument with her sister, {[}Raquel{]}. & Samuel is the \_\_\_\_\_ of Kenneth & \begin{tabular}[c]{@{}l@{}}Kenneth:male,\\ Theresa:female,\\ Ronald:male,\\ Raquel:female,\\ Samuel:male\end{tabular} & 4 & father &  &  \\ \midrule
{[}Steven{]}'s son is {[}Bradford{]}. {[}Bradford{]} and his father always go fishing together on Sundays and have a great time together. {[}Diane{]} is taking her brother {[}Brad{]} out for a late dinner. {[}Kristin{]}, {[}Brad{]}'s mother, is home with a cold. {[}Diane{]}'s father {[}Elmer{]}, and his brother {[}Steven{]}, all got into the rental car to start the long cross-country roadtrip they had been planning. & Bradford is the \_\_\_\_\_ of Kristin & \begin{tabular}[c]{@{}l@{}}Kristin:female,\\ Brad:male,\\ Diane:female,\\ Elmer:male,\\ Steven:male,\\ Bradford:male\end{tabular} & 5 & nephew & 3.78 +- 0.96 &  \\
{[}Elmer{]} went on a roadtrip with his youngest child, {[}Brad{]}. {[}Lena{]} and her sister {[}Diane{]} are going to a restaurant for lunch. {[}Lena{]}'s brother {[}Brad{]} is going to meet them there with his father {[}Elmer{]} {[}Brad{]} ca n't stand his unfriendly aunt {[}Lizzie{]}. & Lizzie is the \_\_\_\_\_ of Diane & \begin{tabular}[c]{@{}l@{}}Diane:female,\\ Lena:female,\\ Brad:male,\\ Elmer:male,\\ Lizzie:female\end{tabular} & 5 & aunt &  &  \\
{[}Ira{]} took his niece {[}April{]} fishing Saturday. They caught a couple small fish. {[}Ronald{]} was enjoying spending time with his fathers, {[}Damion{]} and {[}Claudine{]}. {[}Damion{]} 'other son, {[}Dennis{]}, wanted to come visit too. {[}Dennis{]} often goes out for lunch with his sister, {[}April{]}. & Ira is the \_\_\_\_\_ of Claudine & \begin{tabular}[c]{@{}l@{}}Claudine:female,\\ Ronald:male,\\ Damion:male,\\ Dennis:male,\\ April:female,\\ Ira:male\end{tabular} & 5 & brother &  &  \\ \midrule
{[}Mario{]} wanted to get a good gift for his sister, {[}Marianne{]} {[}Jean{]} and her sister {[}Darlene{]} were going to a party held by {[}Jean{]}'s mom, {[}Marianne{]}. {[}Darlene{]} invited her brother {[}Roy{]} to come, too, but he was too busy. {[}Teri{]} and her father, {[}Mario{]}, had an argument over the weekend. However, they made up by Monday. {[}Agnes{]} wants to make a special meal for her daughter {[}Teri{]}'s birthday. & Roy is the \_\_\_\_\_ of Agnes & \begin{tabular}[c]{@{}l@{}}Agnes:female,\\ Teri:female,\\ Mario:male,\\ Marianne:female,\\ Jean:female,\\ Darlene:female,\\ Roy:male\end{tabular} & 6 & nephew & \multirow{3}{*}{4.46 +- 0.87} &  \\
{[}Robert{]}'s aunt, {[}Marianne{]}, asked {[}Robert{]} to mow the lawn for her. {[}Robert{]} said he could n't because he had a bad back. {[}William{]}'s parents, {[}Brian{]} and {[}Marianne{]}, threw him a surprise party for his birthday. {[}Brian{]}'s daughter {[}Jean{]} made a mental note to be out of town for her birthday! {[}Agnes{]}'s biggest accomplishment is raising her son {[}Robert{]}. {[}Jean{]} is looking for a good gift for her sister {[}Darlene{]}. & Darlene is the \_\_\_\_\_ of Agnes & \begin{tabular}[c]{@{}l@{}}Agnes:female,\\ Robert:male,\\ Marianne:female,\\ William:male,\\ Brian:male,\\ Jean:female,\\ Darlene:female\end{tabular} & 6 & niece &  &  \\
{[}Sharon{]} and her brother {[}Mario{]} went shopping. {[}Teri{]}, {[}Mario{]}'s daughter, came too. {[}Agnes{]}, {[}Annie{]}'s mother, is unhappy with {[}Robert{]}. She feels her son is cruel to {[}Annie{]}'s sister {[}Teri{]}, and she wants {[}Robert{]} to be nicer. {[}Robert{]}'s sister, {[}Nicole{]}, participated in the dance contest. & Nicole is the \_\_\_\_\_ of Sharon & \begin{tabular}[c]{@{}l@{}}Sharon:female,\\ Mario:male,\\ Teri:female,\\ Annie:female,\\ Agnes:female,\\ Robert:male,\\ Nicole:female\end{tabular} & 6 & niece &  &  \\ \bottomrule
\end{tabular}%%
}
\caption{}
\label{tab:my-table}
\end{table*}
